Non-Volatile Memory Accelerated Geometric Multi-Scale Resolution Analysis

Dimensionality reduction algorithms are standard tools in a researcher's toolbox. Dimensionality reduction algorithms are frequently used to augment downstream tasks such as machine learning, data science, and also are exploratory methods for understanding complex phenomena. For instance, dimensionality reduction is commonly used in Biology as well as Neuroscience to understand data collected from biological subjects. However, dimensionality reduction techniques are limited by the von-Neumann architectures that they execute on. Specifically, data intensive algorithms such as dimensionality reduction techniques often require fast, high capacity, persistent memory which historically hardware has been unable to provide at the same time. In this paper, we present a re-implementation of an existing dimensionality reduction technique called Geometric Multi-Scale Resolution Analysis (GMRA) which has been accelerated via novel persistent memory technology called Memory Centric Active Storage (MCAS). Our implementation uses a specialized version of MCAS called PyMM that provides native support for Python datatypes including NumPy arrays and PyTorch tensors. We compare our PyMM implementation against a DRAM implementation, and show that when data fits in DRAM, PyMM offers competitive runtimes. When data does not fit in DRAM, our PyMM implementation is still able to process the data.

==> pymm.tex <==
\subsection{PyMM: Python Micro-MCAS}
PyMM is a new Python library that supports PM. The purpose of PyMM is to ease the use of Python with PM. Thus, PyMM allows running existing data types that are used by numerous libraries in the Python ecosystem.

PyMM is based on the concept of a shelf. A shelf represents a logical grouping of variable instances that are held in a specific set of memory resources. In our case, the resource is a PM, thus the shelves and their variables exist across program runs and machine resets. Variables can also exist outside of any shelf in the DRAM which is also directly attached to the local CPU. A shelf can be created on the two storage types of PM: \emph{devdax} (visible as a character device files) or \emph{fsdax} (visible as block device files).

hey!
just wanted to let you know that I copy-pasted this text into background.tex. I think it makes more sense for it to be there than in this file lol (since the other background text is also in that file)

In our paper we used the shelf type \emph{pymm.ndarray} which is polymorphic with Numpy's \emph{ndarray}. 
This enables Python programmers to run all the functionality of NumPy directly on the PM, functions such as sort, array multiplication, sum. PyMM saves the metadata that allows the program to access the shelf variables in PM. After a crash, the PyMM recovery process is initiated and recovers the metadata that allows the shelf variables to be accessed after a crash.

Under the hood PyMM is using element of MCAS\cite{} for memory allocation and persistency. MCAS is an advanced client-server in-memory object store designed from the ground up to leverage PM.  Micro-MCAS is a local, network-less instantiation of MCAS. Micro-MCAS uses the PM storage components from the fuller MCAS solution.  
